Linear Coding for AWGN channels with Noisy Output Feedback via Dynamic Programming

The optimal coding scheme for communicating a Gaussian message over an Additive White Gaussian noise (AWGN) channel with AWGN output feedback, with a limited number of transmissions is unknown. Even if we restrict the scope of the coding scheme to linear schemes, still, deriving the optimal coding scheme is a challenging task. The state-of-the-art linear scheme for channels with noisy feedback is by Chance and Love, where the coefficients of the linear scheme are numerically optimized based on unique observations [1]. In this paper, we introduce a new class of sequential linear schemes for this channel by introducing a novel linear state process at the transmitter and derive the optimal sequential scheme within this class of schemes in a closed-form by formulating a novel Dynamic Programming (DP). We empirically show that our scheme outperforms the state-of-the-art linear scheme in [1] for noisy feedback and coincides with the SK scheme for noiseless feedback. We also show that in communicating message bits as opposed to a Gaussian message, a learning-based approach further improves the reliability of sequential linear schemes. This problem is an instance of decentralized control without any common information and to the best of our knowledge the first such scenario where we can derive analytical solutions using a DP.

==> GaussianFDBK (2)/0Config.tex <==
%% depending on your installation, you may wish to adjust the top margin:
%\addtolength{\topmargin}{9mm}

%%%%%%
%% Packages:
%% Some useful packages (and compatibility issues with the IEEE format)
%% are pointed out at the very end of this template source file (they are
%% taken verbatim out of bare_conf.tex by Michael Shell).
%
%  Do not adjust lengths that control margins, column widths, etc. 
%  Do not use packages that alter fonts (such as pslatex).         
%
\usepackage{floatrow}
\usepackage{adjustbox}
\usepackage{amsthm}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{ifthen}
\usepackage{cite}
\usepackage{graphicx}
\usepackage[cmex10]{amsmath}
\usepackage{amsfonts,amssymb}
\usepackage{color}
\usepackage{ifthen}
\usepackage{accents}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{listings}
\usepackage{footnote}
\usepackage{array}
\usepackage{verbatim, animate}
\usepackage{comment}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amssymb,latexsym, amsxtra,enumerate}
\usepackage[all]{xy}
\usepackage{psfrag}
\usepackage{xcolor}
\usepackage{lineno}
\usepackage[font=footnotesize]{caption}
\usepackage{multirow}

\usepackage{tikz}
\usetikzlibrary{positioning}
% \include{defns}
\newfloatcommand{capbtabbox}{table}[][\FBwidth]

% \usepackage{auto-pst-pdf}
% \usepackage{pst-pdf}

\newcommand{\bld}[1]{\mathbf{#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\red}[1]{{\color{red}#1}}


\newcommand{\highlight }{\color{blue}}
\newcommand{\Highlight }{\color{red}}
\newcommand{\hk}[1]{\textcolor{purple}{HK: #1}}

\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
  \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
  \addtolength{\dhatheight}{-0.35ex}%
  \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% DEFINITIONS %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cE{\mathcal{E}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\cW{\mathcal{W}}
\def\cP{\mathcal{P}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cR{\mathcal{R}}
\def\cC{\mathcal{C}}
\def\cS{\mathcal{S}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cB{\mathcal{B}}

\def\tw{\tilde{w}}
\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\seq}[1]{\begin{subequations}#1\end{subequations}}
%\newcommand{\eq}[1]{\begin{equation}#1\end{equation}}
\newcommand{\lb}[1]{\left\{ \begin{array}{ll} #1 \end{array} \right.}
\newcommand\dif{\mathop{}\!\mathrm{d}}
\newcommand{\bm}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bit}[1]{\begin{itemize}#1\end{itemize}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\sect}[1]{Section~\ref{#1}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\mE}{\mathbb{E}}
\newcommand{\mR}{\mathbb{R}}

\newcommand{\sq}[1]{\left[#1\right]}
\newcommand{\cq}[1]{\left(#1\right)}
\newcommand{\bq}[1]{\left\{#1\right\}}

\newcommand{\tcC}{\tilde{\mathcal{C}}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hN}{\hat{N}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\hz}{\hat{z}}
\newcommand{\hw}{\hat{w}}
\newcommand{\ha}{\hat{a}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hcC}{\hat{\mathcal{C}}}
\newcommand{\hD}{\hat{D}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\gtt}{\gamma_{t+1}}
\newcommand{\tgamma}{\tilde{\phi}}
\newcommand{\Qx}[1]{Q^{i}(#1)}
\newcommand{\Qw}[1]{Q_w^{i}(#1)}
\newcommand{\apos}{\textsc{\char13}}


\newcommand{\pushright}[1]{\ifmeasuring@ #1 \else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@ #1 \else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\newcommand{\nn}{\nonumber}
\newcommand{\rd}{\right.}
\newcommand{\ld}{\left.}

\newcommand{\phienc}{\phi_{t}^{\mathrm{enc}}}
\newcommand{\psidec}{\psi^{\mathrm{dec}}}
\newcommand{\at}{\tilde{a}}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\sut}{\sigma_{u,t}}
\newcommand{\sutt}{\sigma_{u,t+1}}

\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}


\newcommand{\ve}[1]{\underline{#1}}
\newcommand{\eqdef}{\stackrel{\scriptscriptstyle \triangle}{=}}
\newcommand{\mdef}{\stackrel{\text{\tiny def}}{=}}
\def\Real{\mathbb{R}}
\def\P{\mathbb{P}}



%% Mathcal (discrete sets)
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\cc}{\text{\footnotesize $\mathcal{C}$} }
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mspace{1.5mu}\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


\DeclareMathOperator\E{\textsf{E}}

\def\cE{\mathcal{E}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\cW{\mathcal{W}}
\def\cP{\mathcal{P}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cR{\mathcal{R}}
\def\cC{\mathcal{C}}
\def\cS{\mathcal{S}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cB{\mathcal{B}}

\def\tw{\tilde{w}}
\def\gt{\gamma_t}
%\newcommand{\eq}[1]{\begin{equation}#1\end{equation}}

\def\Real{\mathbb{R}}
\def\P{\mathbb{P}}


\makeatletter
\newcommand{\printfnsymbol}[1]{%
  \textsuperscript{\@fnsymbol{#1}}%
}
\makeatother



%% Hats
\newcommand{\Kh}{{\hat{K}}}
\newcommand{\Lh}{{\hat{L}}}
\newcommand{\Mh}{{\hat{M}}}
\newcommand{\Rh}{{\hat{R}}}
\newcommand{\Sh}{{\hat{S}}}
\newcommand{\Uh}{{\hat{U}}}
\newcommand{\Vh}{{\hat{V}}}
\newcommand{\Wh}{{\hat{W}}}
\newcommand{\Xh}{{\hat{X}}}
\newcommand{\Yh}{{\hat{Y}}}
\newcommand{\Zh}{{\hat{Z}}}
\renewcommand{\dh}{{\hat{d}}}
\newcommand{\kh}{{\hat{k}}}
\newcommand{\lh}{{\hat{l}}}
\newcommand{\mh}{{\hat{m}}}
\newcommand{\sh}{{\hat{s}}}
\newcommand{\uh}{{\hat{u}}}
\newcommand{\vh}{{\hat{v}}}
\newcommand{\wh}{{\hat{w}}}
\newcommand{\xh}{{\hat{x}}}
\newcommand{\yh}{{\hat{y}}}
\newcommand{\zh}{{\hat{z}}}
\newcommand{\gh}{{\hat{g}}}
%% Tildes
\newcommand{\At}{{\tilde{A}}}
\newcommand{\Ct}{{\tilde{C}}}
\newcommand{\Kt}{{\tilde{K}}}
\newcommand{\Lt}{{\tilde{L}}}
\newcommand{\Mt}{{\tilde{M}}}
\newcommand{\Nt}{{\tilde{N}}}
\newcommand{\Qt}{{\tilde{Q}}}
\newcommand{\Rt}{{\tilde{R}}}
\newcommand{\St}{{\tilde{S}}}
\newcommand{\Ut}{{\tilde{U}}}
\newcommand{\Vt}{{\tilde{V}}}
\newcommand{\Wt}{{\tilde{W}}}
\newcommand{\Xt}{{\tilde{X}}}
\newcommand{\Yt}{{\tilde{Y}}}
\newcommand{\Zt}{{\tilde{Z}}}
\newcommand{\dt}{{\tilde{d}}}
\newcommand{\kt}{{\tilde{k}}}
\newcommand{\lt}{{\tilde{l}}}
\newcommand{\mt}{{\tilde{m}}}
\newcommand{\pt}{{\tilde{p}}}
\newcommand{\rt}{{\tilde{r}}}
\newcommand{\st}{{\tilde{s}}}
\newcommand{\ut}{{\tilde{u}}}
\newcommand{\vt}{{\tilde{v}}}
\newcommand{\wt}{{\tilde{w}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\yt}{{\tilde{y}}}
\newcommand{\zt}{{\tilde{z}}}
\newcommand{\nt}{{\tilde{n}}}

==> GaussianFDBK (2)/0Glossary.tex <==
\usepackage{xspace}
\usepackage[acronym,nogroupskip,nonumberlist,nopostdot]{glossaries}

\newacronym{mdp}{MDP}{Markov decision process}
\newacronym{ne}{NE}{Nash equillibrium}
\newacronym{mfe}{MFE}{mean-field equillibrium}
\newacronym{mpe}{MPE}{Markov perfect equillibrium}
\newacronym{mfg}{MFG}{mean-field game}
\newacronym{rl}{RL}{reinforcement learning}
\newacronym{marl}{MARL}{multi-agent reinforcement learning}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{ssg}{SSG}{Stackelberg Security Game}
\newacronym{pse}{PSE}{Perfect Stackelberg Equilibrium}
\newacronym{mpse}{MPSE}{Markov \gls{pse}}
\newacronym{spbe}{SPBE}{Sub-game Perfect Bayesian Equilibrium}
\newacronym{pf}{PF}{particle filter}
\newacronym{pomdp}{POMDP}{partially obseravable \gls{mdp}}
\newacronym{nn}{NN}{neural network}
\newacronym{td}{TD}{Temporal Difference}
\newacronym{awgn}{AWGN}{Additive White Gaussian noise}
\newacronym{tim}{TIM}{topological interference management}
\newacronym{gdof}{GDoF}{generalized degrees of freedom}
\newacronym{snr}{SNR}{Signal to Noise Ratio}
\newacronym{sinr}{SINR}{signal to noise and interference ratio}
\newacronym{inr}{INR}{interference to noise ratio}
\newacronym{pam}{PAM}{Pulse Amplitude Modulation}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{ber}{BER}{Bit Error Rate}
\newacronym{tdm}{TDM}{time domain multiplexing}
\newacronym{gan}{GAN}{Generative Adversarial Network}
\newacronym{sir}{SIR}{signal to interference ratio}
\newacronym{mmse}{MMSE}{Minimum Mean-squared error}
\newacronym{sk}{SK}{Schalkwijk-Kailath}
\newacronym{bsc}{BSC}{binary symmetric channel}
\newacronym{ldpc}{LDPC}{low density parity codes}
\newacronym{ml}{ML}{maximum likelihood}
\newacronym{dp}{DP}{Dynamic Programming}
\newacronym{rnn}{RNN}{Recurrent Neural Network}
\newacronym{cdf}{CDF}{Cummulative Distribution Function}
\newacronym{cl}{CL}{Chance and Love}

\newcommand{\cl}{\gls{cl}\xspace}
\newcommand{\rnn}{\gls{rnn}\xspace}
\newcommand{\dpp}{\gls{dp}\xspace}
\newcommand{\ml}{\gls{ml}\xspace}
\newcommand{\ldpc}{\gls{ldpc}\xspace}
\newcommand{\bsc}{\gls{bsc}\xspace}
\newcommand{\sk}{\gls{sk}\xspace}
\newcommand{\mdp}{\gls{mdp}\xspace}
\newcommand{\gne}{\gls{ne}\xspace}
\newcommand{\mfe}{\gls{mfe}\xspace}
\newcommand{\mpe}{\gls{mpe}\xspace}
\newcommand{\mfg}{\gls{mfg}\xspace}
\newcommand{\mfgs}{\glspl{mfg}\xspace}
\newcommand{\rl}{\gls{rl}\xspace}
\newcommand{\marl}{\gls{marl}\xspace}
\newcommand{\ssg}{\gls{ssg}\xspace}
\newcommand{\ssgs}{\glspl{ssg}\xspace}
\newcommand{\pse}{\gls{pse}\xspace}
\newcommand{\mpse}{\gls{mpse}\xspace}
\newcommand{\spbe}{\gls{spbe}\xspace}
\newcommand{\pf}{\gls{pf}\xspace}
\newcommand{\pomdp}{\glspl{pomdp}\xspace}
\newcommand{\neural}{\gls{nn}\xspace}
\newcommand{\td}{\gls{td}\xspace}
\newcommand{\awgn}{\gls{awgn}\xspace}
\newcommand{\tim}{\gls{tim}\xspace}
\newcommand{\gdof}{\gls{gdof}\xspace}
\newcommand{\snr}{\gls{snr}\xspace}
\newcommand{\sinr}{\gls{sinr}\xspace}
\newcommand{\inr}{\gls{inr}\xspace}
\newcommand{\pam}{\gls{pam}\xspace}
\newcommand{\mse}{\gls{mse}\xspace}
\newcommand{\ber}{\gls{ber}\xspace}
\newcommand{\tdm}{\gls{tdm}\xspace}
\newcommand{\gan}{\gls{gan}\xspace}
\newcommand{\sir}{\gls{sir}\xspace}
\newcommand{\mmse}{\gls{mmse}\xspace}
\newcommand{\cdf}{\gls{cdf}\xspace}

==> GaussianFDBK (2)/defns.tex <==
%% 
%% Common definitions
%% Only contains the definitions, not formatting information
%%

\usepackage{xspace}
\usepackage{bbm}
<<<<<<< HEAD
% \input{mathlig}
=======
\input{mathlig}
>>>>>>> 0dffceb9eb5ee636555f67a2992b801d7336bc19

%% |
\DeclareRobustCommand{\scond}{\mathchoice{\muspace\vert\muspace}{\vert}{\vert}{\vert}}
\mathlig{|}{\scond}

%% :
\DeclareRobustCommand{\discint}{\mathchoice{\mspace{-1.5mu}:\mspace{-1.5mu}}{\mspace{-1.5mu}:\mspace{-1.5mu}}{:}{:}}
\mathlig{::}{\discint}

%% A few operator definitions
\def\tr{\mathop{\rm tr}\nolimits}%
\def\var{\mathop{\rm Var}\nolimits}%
\def\Var{\mathop{\rm Var}\nolimits}%
\def\cov{\mathop{\rm Cov}\nolimits}%
\def\Cov{\mathop{\rm Cov}\nolimits}%
\def\diag{\mathop{\rm diag}\nolimits}%
\def\Re{\mathop{\rm Re}\nolimits}%
\def\Im{\mathop{\rm Im}\nolimits}%
\def\rank{\mathop{\rm rank}\nolimits}%
\def\essinf{\mathop{\rm ess\,inf}}%
\def\sgn{\mathop{\rm sgn}\nolimits}%
\def\erfc{\mathop{\rm erfc}\nolimits}%
\def\co{\mathop{\rm co}\nolimits}%





%% Script sets: Capacity region, set of probs, achievable rate region, etc.

\renewcommand{\Pr}{\mathscr{P}}

%% Sequences
%% TODO: Should be cleaned up
\iffalse
  \newcommand{\Un}{{U_1,U_2,\ldots,U_n}}
  \newcommand{\Vn}{{V_1,V_2,\ldots,V_n}}
  \newcommand{\Xk}{{X^{(1)},X^{(2)},\ldots,X^{(k)}}}
  \newcommand{\xk}{{x^{(1)},x^{(2)},\ldots,x^{(k)}}}
  \newcommand{\Xm}{{X^{(1)},X^{(2)},\ldots,X^{(m)}}}
  \newcommand{\xm}{{x^{(1)},x^{(2)},\ldots,x^{(m)}}}
  \newcommand{\Xn}{{X_1,X_2,\ldots,X_n}}
  \newcommand{\xn}{{x_1,x_2,\ldots,x_n}}
  \newcommand{\Ym}{{Y^{(1)},Y^{(2)},\ldots,Y^{(m)}}}
  \newcommand{\ym}{{y^{(1)},y^{(2)},\ldots,y^{(m)}}}
  \newcommand{\Yn}{{Y_1,Y_2,\ldots,Y_n}}
  \newcommand{\yn}{{y_1,y_2,\ldots,y_n}}
  \newcommand{\Zn}{{Z_1,Z_2,\ldots,Z_n}}
  \newcommand{\zn}{{z_1,z_2,\ldots,z_n}}
\fi


%% Boldface vectors
%%




\renewcommand{\dh}{{\hat{d}}}

%% 
%% Greek
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\l{\lambda}
\def\th{\theta}
\def\Th{\Theta}


\let\P\relax
\DeclareMathOperator\P{\textsf{P}}


%\DeclareMathOperator\C{C}
%\DeclareMathOperator\R{R}

%% Error symbol
\def\error{\mathrm{e}}

%% Probability distributions
%%\newcommand{\Br}{\mathrm{Bern}}

%%\newcommand{\Norm}{\mathrm{N}}

%% Misc
\newcommand\eg{e.g.,\xspace}
\newcommand\ie{i.e.,\xspace}
\def\textiid{i.i.d.\@\xspace}
\newcommand\iid{\ifmmode\text{ i.i.d. } \else \textiid \fi}
\let\textand\and
%\renewcommand\and{\ifmmode{\text{ and }}{\textand}}
\let\textor\or
%\renewcommand\or{\ifmmode{\text{ or }}{\textor}}
\newcommand{\geql}{\succeq}
\newcommand{\leql}{\preceq}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Ff}{\mathbb{F}}
\newcommand{\Zz}{\mathbb{Z}}
\newcommand{\ind}{\boldsymbol{1}}
\newcommand{\defeq}{=}
\newcommand{\carddot}{\mathchoice{\!\cdot\!}{\!\cdot\!}{\cdot}{\cdot}}

%%------------------------------------------------------- 
%% Fractions
%%
\newcommand{\sfrac}[2]{\mbox{\small$\displaystyle\frac{#1}{#2}$}}
\newcommand{\half}{\sfrac{1}{2}}

%%------------------------------------------------------- 
%% Cups and caps
%%
\def\medcupmath{\mbox{\small$\displaystyle\bigcup$}}
\def\medcuptext{\raisebox{1pt}{\small$\textstyle\bigcup$}}
\def\medcup{\mathop{\mathchoice{\medcupmath}{\medcuptext}{\bigcup}{\bigcup}}}

\def\medcapmath{\raisebox{0.5pt}{\small$\displaystyle\bigcap$}}
\def\medcaptext{\raisebox{1pt}{\small$\textstyle\bigcap$}}
\def\medcap{\mathop{\mathchoice{\medcapmath}{\medcaptext}{\bigcap}{\bigcap}}}


%%------------------------------------------------------- 
%% Products
%%
\def\medtimesmath{\mbox{\small$\displaystyle\bigtimes$}}
\def\medtimestext{\raisebox{1pt}{\small$\textstyle\bigtimes$}}
\def\medtimes{\mathop{\mathchoice{\medtimesmath}{\medtimestext}{\bigtimes}{\bigtimes}}}


%%--------------------------------------------------------
%% Spacing
%%
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathllapinternal#1#2{%
\llap{$\mathsurround=0pt#1{#2}$}}

\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathrlapinternal#1#2{%
\rlap{$\mathsurround=0pt#1{#2}$}}

\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathclapinternal#1#2{%
\clap{$\mathsurround=0pt#1{#2}$}}

%% For lecture notes
\def\labelitemi{$\bullet$}
\def\labelitemii{$\bullet$}
%\def\labelitemii{$\circ$}

%%-------------------------------------------------------
%% Stackrel
%%

\let\oldstackrel\stackrel
\renewcommand{\stackrel}[2]{\oldstackrel{\mathclap{#1}}{#2}}

%-------------------------------------------------------------------------
% Interchapter macros

\newcommand{\Csum}{C_\mathrm{sum}}
\newcommand{\Csym}{C_\mathrm{sym}}
\newcommand{\Ccc}{C_\mathrm{CC}}
\newcommand{\Cavc}{C_\mathrm{AVC}}
\newcommand{\Cnsi}{C_\mathrm{NSI}}
\newcommand{\CXX}[3]{{#1}_{\mathrm{#2\text{-}#3}}}
\newcommand{\Csid}{\CXX{C}{SI}{D}}
\newcommand{\Csie}{\CXX{C}{SI}{E}}
\newcommand{\Csied}{\CXX{C}{SI}{ED}}
\newcommand{\Ccsie}{\CXX{C}{CSI}{E}}
\newcommand{\Crsid}{\CXX{\Cr}{SI}{D}}
\newcommand{\Crsied}{\CXX{\Cr}{SI}{ED}}
\newcommand{\Crdsied}{\CXX{\Cr}{DSI}{ED}}

\newcommand{\Rsid}{\CXX{R}{SI}{D}}
\newcommand{\Rcsid}{\CXX{R}{CSI}{D}}
\newcommand{\Rcsied}{\CXX{R}{CSI}{ED}}
\newcommand{\Rsied}{\CXX{R}{SI}{ED}}
\newcommand{\Rsie}{\CXX{R}{SI}{E}}

\newcommand{\Rs}{R_\mathrm{s}}
\newcommand{\Ms}{M_\mathrm{s}}
\newcommand{\ms}{m_\mathrm{s}}
\newcommand{\mk}{m_\mathrm{K}}

\newcommand{\Rcfo}{R_\mathrm{CFO}}
\newcommand{\Rrcfo}{\Rr_\mathrm{CFO}}
\newcommand{\Cs}{C_\mathrm{S}}
\newcommand{\Ck}{C_\mathrm{K}}
\newcommand{\Rk}{R_\mathrm{K}}
\newcommand{\Rl}{R_\mathrm{L}}
\newcommand{\Rln}{R_\mathrm{L}^{(n)}}
\newcommand{\Ckone}{C_\mathrm{K}^{(1)}}
\newcommand{\Ckq}{C_\mathrm{K}^{(q)}}
\newcommand{\Ckow}{\CXX{C}{K}{OW}}
\newcommand{\Ckcm}{\CXX{C}{K}{CM}}

\newcommand{\musum}{$\muv$\nobreakdash-sum}
%-------------------------------------------------------------------------
% PSFrag vertical adjustment

\newcommand{\adjas}[2]{\smash{#1}\vphantom{#2}}
\newcommand{\adjasm}[1]{\adjas{#1}{$m$}}
\newcommand{\adjasM}[1]{\adjas{#1}{$M$}}

%-------------------------------------------------------------------------
% Overline
\newcommand{\Hbar}{H\mathllap{\overline{\vphantom{H}\hphantom{\rule{6.9pt}{0pt}}}\mspace{0.7mu}}}
\newcommand{\Gbar}{G\mathllap{\overline{\vphantom{G}\hphantom{\rule{6.25pt}{0pt}}}\mspace{1.1mu}}}
\renewcommand{\hbar}{h\mathllap{\overline{\vphantom{h}\hphantom{\rule{4.6pt}{0pt}}}\mspace{0.77mu}}}

%------------------------------------
% URL tilde
\catcode`~=11 % make LaTeX treat tilde (~) like a normal character
\newcommand{\urltilde}{\kern -.06em\lower -.06em\hbox{~}\kern .02em}
\catcode`~=13 % revert back to treating tilde (~) as an active character


%------------------------------------
% Hyphenation
\hyphenation{Gauss-ian}
\hyphenation{qua-dra-tic}
\hyphenation{Vis-wa-nath}
\hyphenation{non-trivial}
\hyphenation{multi-letter}
\hyphenation{Gauss-ian}
\hyphenation{super-posi-tion}
\hyphenation{de-cod-er}
\hyphenation{Nara-yan}
\hyphenation{multi-message}
\hyphenation{Dimi-tris}
\hyphenation{Pol-ty-rev}
\hyphenation{multi-cast}
\hyphenation{multi-user}
\hyphenation{multi-plex-ing}
\hyphenation{bi-directional}
\hyphenation{comput}

==> defns.tex <==
%% 
%% Common definitions
%% Only contains the definitions, not formatting information
%%

\usepackage{xspace}
\usepackage{bbm}
<<<<<<< HEAD
% \input{mathlig}
=======
\input{mathlig}
>>>>>>> 0dffceb9eb5ee636555f67a2992b801d7336bc19

%% |
\DeclareRobustCommand{\scond}{\mathchoice{\muspace\vert\muspace}{\vert}{\vert}{\vert}}
\mathlig{|}{\scond}

%% :
\DeclareRobustCommand{\discint}{\mathchoice{\mspace{-1.5mu}:\mspace{-1.5mu}}{\mspace{-1.5mu}:\mspace{-1.5mu}}{:}{:}}
\mathlig{::}{\discint}

%% A few operator definitions
\def\tr{\mathop{\rm tr}\nolimits}%
\def\var{\mathop{\rm Var}\nolimits}%
\def\Var{\mathop{\rm Var}\nolimits}%
\def\cov{\mathop{\rm Cov}\nolimits}%
\def\Cov{\mathop{\rm Cov}\nolimits}%
\def\diag{\mathop{\rm diag}\nolimits}%
\def\Re{\mathop{\rm Re}\nolimits}%
\def\Im{\mathop{\rm Im}\nolimits}%
\def\rank{\mathop{\rm rank}\nolimits}%
\def\essinf{\mathop{\rm ess\,inf}}%
\def\sgn{\mathop{\rm sgn}\nolimits}%
\def\erfc{\mathop{\rm erfc}\nolimits}%
\def\co{\mathop{\rm co}\nolimits}%





%% Script sets: Capacity region, set of probs, achievable rate region, etc.

\renewcommand{\Pr}{\mathscr{P}}

%% Sequences
%% TODO: Should be cleaned up
\iffalse
  \newcommand{\Un}{{U_1,U_2,\ldots,U_n}}
  \newcommand{\Vn}{{V_1,V_2,\ldots,V_n}}
  \newcommand{\Xk}{{X^{(1)},X^{(2)},\ldots,X^{(k)}}}
  \newcommand{\xk}{{x^{(1)},x^{(2)},\ldots,x^{(k)}}}
  \newcommand{\Xm}{{X^{(1)},X^{(2)},\ldots,X^{(m)}}}
  \newcommand{\xm}{{x^{(1)},x^{(2)},\ldots,x^{(m)}}}
  \newcommand{\Xn}{{X_1,X_2,\ldots,X_n}}
  \newcommand{\xn}{{x_1,x_2,\ldots,x_n}}
  \newcommand{\Ym}{{Y^{(1)},Y^{(2)},\ldots,Y^{(m)}}}
  \newcommand{\ym}{{y^{(1)},y^{(2)},\ldots,y^{(m)}}}
  \newcommand{\Yn}{{Y_1,Y_2,\ldots,Y_n}}
  \newcommand{\yn}{{y_1,y_2,\ldots,y_n}}
  \newcommand{\Zn}{{Z_1,Z_2,\ldots,Z_n}}
  \newcommand{\zn}{{z_1,z_2,\ldots,z_n}}
\fi


%% Boldface vectors
%%




\renewcommand{\dh}{{\hat{d}}}

%% 
%% Greek
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\l{\lambda}
\def\th{\theta}
\def\Th{\Theta}


\let\P\relax
\DeclareMathOperator\P{\textsf{P}}


%\DeclareMathOperator\C{C}
%\DeclareMathOperator\R{R}

%% Error symbol
\def\error{\mathrm{e}}

%% Probability distributions
%%\newcommand{\Br}{\mathrm{Bern}}

%%\newcommand{\Norm}{\mathrm{N}}

%% Misc
\newcommand\eg{e.g.,\xspace}
\newcommand\ie{i.e.,\xspace}
\def\textiid{i.i.d.\@\xspace}
\newcommand\iid{\ifmmode\text{ i.i.d. } \else \textiid \fi}
\let\textand\and
%\renewcommand\and{\ifmmode{\text{ and }}{\textand}}
\let\textor\or
%\renewcommand\or{\ifmmode{\text{ or }}{\textor}}
\newcommand{\geql}{\succeq}
\newcommand{\leql}{\preceq}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Ff}{\mathbb{F}}
\newcommand{\Zz}{\mathbb{Z}}
\newcommand{\ind}{\boldsymbol{1}}
\newcommand{\defeq}{=}
\newcommand{\carddot}{\mathchoice{\!\cdot\!}{\!\cdot\!}{\cdot}{\cdot}}

%%------------------------------------------------------- 
%% Fractions
%%
\newcommand{\sfrac}[2]{\mbox{\small$\displaystyle\frac{#1}{#2}$}}
\newcommand{\half}{\sfrac{1}{2}}

%%------------------------------------------------------- 
%% Cups and caps
%%
\def\medcupmath{\mbox{\small$\displaystyle\bigcup$}}
\def\medcuptext{\raisebox{1pt}{\small$\textstyle\bigcup$}}
\def\medcup{\mathop{\mathchoice{\medcupmath}{\medcuptext}{\bigcup}{\bigcup}}}

\def\medcapmath{\raisebox{0.5pt}{\small$\displaystyle\bigcap$}}
\def\medcaptext{\raisebox{1pt}{\small$\textstyle\bigcap$}}
\def\medcap{\mathop{\mathchoice{\medcapmath}{\medcaptext}{\bigcap}{\bigcap}}}


%%------------------------------------------------------- 
%% Products
%%
\def\medtimesmath{\mbox{\small$\displaystyle\bigtimes$}}
\def\medtimestext{\raisebox{1pt}{\small$\textstyle\bigtimes$}}
\def\medtimes{\mathop{\mathchoice{\medtimesmath}{\medtimestext}{\bigtimes}{\bigtimes}}}


%%--------------------------------------------------------
%% Spacing
%%
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathllapinternal#1#2{%
\llap{$\mathsurround=0pt#1{#2}$}}

\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathrlapinternal#1#2{%
\rlap{$\mathsurround=0pt#1{#2}$}}

\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathclapinternal#1#2{%
\clap{$\mathsurround=0pt#1{#2}$}}

%% For lecture notes
\def\labelitemi{$\bullet$}
\def\labelitemii{$\bullet$}
%\def\labelitemii{$\circ$}

%%-------------------------------------------------------
%% Stackrel
%%

\let\oldstackrel\stackrel
\renewcommand{\stackrel}[2]{\oldstackrel{\mathclap{#1}}{#2}}

%-------------------------------------------------------------------------
% Interchapter macros

\newcommand{\Csum}{C_\mathrm{sum}}
\newcommand{\Csym}{C_\mathrm{sym}}
\newcommand{\Ccc}{C_\mathrm{CC}}
\newcommand{\Cavc}{C_\mathrm{AVC}}
\newcommand{\Cnsi}{C_\mathrm{NSI}}
\newcommand{\CXX}[3]{{#1}_{\mathrm{#2\text{-}#3}}}
\newcommand{\Csid}{\CXX{C}{SI}{D}}
\newcommand{\Csie}{\CXX{C}{SI}{E}}
\newcommand{\Csied}{\CXX{C}{SI}{ED}}
\newcommand{\Ccsie}{\CXX{C}{CSI}{E}}
\newcommand{\Crsid}{\CXX{\Cr}{SI}{D}}
\newcommand{\Crsied}{\CXX{\Cr}{SI}{ED}}
\newcommand{\Crdsied}{\CXX{\Cr}{DSI}{ED}}

\newcommand{\Rsid}{\CXX{R}{SI}{D}}
\newcommand{\Rcsid}{\CXX{R}{CSI}{D}}
\newcommand{\Rcsied}{\CXX{R}{CSI}{ED}}
\newcommand{\Rsied}{\CXX{R}{SI}{ED}}
\newcommand{\Rsie}{\CXX{R}{SI}{E}}

\newcommand{\Rs}{R_\mathrm{s}}
\newcommand{\Ms}{M_\mathrm{s}}
\newcommand{\ms}{m_\mathrm{s}}
\newcommand{\mk}{m_\mathrm{K}}

\newcommand{\Rcfo}{R_\mathrm{CFO}}
\newcommand{\Rrcfo}{\Rr_\mathrm{CFO}}
\newcommand{\Cs}{C_\mathrm{S}}
\newcommand{\Ck}{C_\mathrm{K}}
\newcommand{\Rk}{R_\mathrm{K}}
\newcommand{\Rl}{R_\mathrm{L}}
\newcommand{\Rln}{R_\mathrm{L}^{(n)}}
\newcommand{\Ckone}{C_\mathrm{K}^{(1)}}
\newcommand{\Ckq}{C_\mathrm{K}^{(q)}}
\newcommand{\Ckow}{\CXX{C}{K}{OW}}
\newcommand{\Ckcm}{\CXX{C}{K}{CM}}

\newcommand{\musum}{$\muv$\nobreakdash-sum}
%-------------------------------------------------------------------------
% PSFrag vertical adjustment

\newcommand{\adjas}[2]{\smash{#1}\vphantom{#2}}
\newcommand{\adjasm}[1]{\adjas{#1}{$m$}}
\newcommand{\adjasM}[1]{\adjas{#1}{$M$}}

%-------------------------------------------------------------------------
% Overline
\newcommand{\Hbar}{H\mathllap{\overline{\vphantom{H}\hphantom{\rule{6.9pt}{0pt}}}\mspace{0.7mu}}}
\newcommand{\Gbar}{G\mathllap{\overline{\vphantom{G}\hphantom{\rule{6.25pt}{0pt}}}\mspace{1.1mu}}}
\renewcommand{\hbar}{h\mathllap{\overline{\vphantom{h}\hphantom{\rule{4.6pt}{0pt}}}\mspace{0.77mu}}}

%------------------------------------
% URL tilde
\catcode`~=11 % make LaTeX treat tilde (~) like a normal character
\newcommand{\urltilde}{\kern -.06em\lower -.06em\hbox{~}\kern .02em}
\catcode`~=13 % revert back to treating tilde (~) as an active character


%------------------------------------
% Hyphenation
\hyphenation{Gauss-ian}
\hyphenation{qua-dra-tic}
\hyphenation{Vis-wa-nath}
\hyphenation{non-trivial}
\hyphenation{multi-letter}
\hyphenation{Gauss-ian}
\hyphenation{super-posi-tion}
\hyphenation{de-cod-er}
\hyphenation{Nara-yan}
\hyphenation{multi-message}
\hyphenation{Dimi-tris}
\hyphenation{Pol-ty-rev}
\hyphenation{multi-cast}
\hyphenation{multi-user}
\hyphenation{multi-plex-ing}
\hyphenation{bi-directional}
\hyphenation{comput}
